CBR-RAG: Case-Based Reasoning for Retrieval Augmented Generation in LLMs for Legal Question Answering

Retrieval-Augmented Generation (RAG) enhances Large Language Model (LLM) output by providing prior knowledge as context to input. This is beneficial for knowledge-intensive and expert reliant tasks, including legal question-answering, which require evidence to validate generated text outputs. We highlight that Case-Based Reasoning (CBR) presents key opportunities to structure retrieval as part of the RAG process in an LLM. We introduce CBR-RAG, where CBR cycle's initial retrieval stage, its indexing vocabulary, and similarity knowledge containers are used to enhance LLM queries with contextually relevant cases. This integration augments the original LLM query, providing a richer prompt. We present an evaluation of CBR-RAG, and examine different representations (i.e. general and domain-specific embeddings) and methods of comparison (i.e. inter, intra and hybrid similarity) on the task of legal question-answering. Our results indicate that the context provided by CBR's case reuse enforces similarity between relevant components of the questions and the evidence base leading to significant improvements in the quality of generated answers.

==> tex-scratch <==
\begin{table}[!htb]
\centering
\renewcommand{\arraystretch}{1.2}
\caption{Cosine scores for hybrid algorithms against $k$}
\begin{tabular}{@{\hspace{5pt}} l @{\hspace{10pt}} l @{\hspace{5pt}} l @{\hspace{5pt}} r @{\hspace{5pt}}}
\toprule
$k$ & Algorithm & LLM Context & Cosine \\
\midrule
0 & No-RAG & -- & 0.8967 \\
\midrule
\multirow{6}{*}{1} & \multirow{2}{*}{Hybrid BERT} & snippet & 0.8986 \\
& & full case & 0.9068 \\
\cline{2-4}
& \multirow{2}{*}{Hybrid LBERT} & snippet & 0.9020 \\
& & full case & 0.9043 \\
\cline{2-4}
& \multirow{2}{*}{Hybrid ABERT} & snippet & 0.9121 \\
& & full case & 0.9074 \\
\midrule
\multirow{6}{*}{3} & \multirow{2}{*}{Hybrid BERT} & snippet & 0.9007 \\
& & full case & 0.8998 \\
\cline{2-4}
& \multirow{2}{*}{Hybrid LBERT} & snippet & 0.9034 \\
& & full case & 0.9045 \\
\cline{2-4}
& \multirow{2}{*}{Hybrid ABERT} & snippet & 0.9092\\
& & full case & \textbf{0.9141} \\
\bottomrule
\end{tabular}
\label{tab:addlabel}
\end{table}

\begin{table}[htbp]
\centering
\renewcommand{\arraystretch}{1.2}
\caption{Prompts Used in this research.}
\begin{tabular}{@{}p{0.20\linewidth}p{0.19\linewidth}p{0.60\linewidth}@{}}
\toprule
\textbf{Scenario} & \textbf{Used LLM} & \textbf{Prompt} \\
\midrule
Extracting legal acts from texts. & Gpt-3.5-turbo-0125 & Extract the legal act(s) in this text. Print 'None' if nothing is found. \{ TEXT \} \\ 
\midrule
Extracting entities / unique identifiers from texts. & Gpt-3.5-turbo-0125 & Extract named entities and unique identifiers as a single text (separated with white-space) line from this " + TEXT. Print '' if nothing is found. \{ TEXT \} \\ 
\midrule
Generating questions from text pairs. & Mistral-7b & Produce a question and answer where the answer requires detailed access to both Text 1 and Text 2. Don’t refer texts in the question or answer. \{ Text1: TEXT1 — Text2: TEXT \} \\ 
\midrule
Generating output from snippets. & Mistral-7b & Answer QUESTION by using the following contexts: \{ TEXT1 — TEXT2 \} \\ 
\midrule
Generating Mistral output from cases. & Mistral-7b & Answer QUESTION as a simple string (with no structure) by using the following question, citation, and answer tuples as context: \{ Question: Q1, Citation: C1, Answer: A1 — Question: Q2, Citation: C2, Answer: A2 \} \\
\bottomrule
\end{tabular}
\label{tab:scenarios-prompts}
\end{table}

We define the algorithms based on their embedding strategy ($f$ for \emph{Intra}, $g$ for \emph{Inter}, $h$ for \emph{Hybrid}) and the scope of case information used (\(S\) for support part, \(C\) for full case):


\begin{enumerate}
\item \cbrragFS and \cbrragFCase both use intra-embedding, with \cbrragFS utilising the support part of the retrieved case (Refer equations~\ref{eq:intra} and~\ref{eq:support}) and \cbrragFCase using the full case. (Refer equations~\ref{eq:intra} and~\ref{eq:case}).
%\item \cbrragFCase Intra-embedding, using the full case context (Refer equations~\ref{eq:intra} and~\ref{eq:case}).
\item \cbrragGS and \cbrragGCase both use inter-embedding, with \cbrragGS using the support part of the retrieved case (Refer equations~\ref{eq:inter} and~\ref{eq:support}), and
\cbrragGCase using the full retrieved case (Refer equations~\ref{eq:inter} and~\ref{eq:case}).
\item \cbrragGES and \cbrragGECase, similar to above except Inter-embeddings on the entity part of the case used for retrieval.  (Refer equations~\ref{eq:inter} and~\ref{eq:case}).
\item \cbrragHS and \cbrragHCase adopts the hybrid embedding, with \cbrragHS using the support part of the retrieved case (Refer equations~\ref{eq:hybrid} and~\ref{eq:support}), 
and \cbrragHCase using the full retrieved case (Refer equations~\ref{eq:hybrid} and~\ref{eq:case}).
%\item \cbrragHCase Hybrid embedding, using the full case context (Refer equations~\ref{eq:hybrid} and~\ref{eq:case}).
\end{enumerate}

%CBR para
%
%In Textual CBR, a key focus has been on extracting features for case comparison, employing methods that range from decision trees, as exemplified by the SMILE system in creating indexing vocabularies for legal case retrieval~\cite{bruninghaus2001role}, to the use of association rules for case representation~\cite{wiratunga-2004}. Much of which has now been taken over by neural transformations of input text by transformer style mebeddings. 

%In the SMILE system, an indexing vocabulary was created automatically by learning decision tree-like structure, facilitating case retrieval thought tree traversal~\cite{bruninghaus2001role}. More generally research in Textual CBR has predominantly focused on extracting textual features to navigate the challenges posed by synonymy and polysemy, thereby developing semantic concepts to be used for case comparison~\cite{wiratunga-2004}.


Finding datasets large enough to train LLMs is another challenge. 
Typically, these transformers are pre-trained on general text, and later fine-tuned using legal text classification downstream tasks to learn domain-specific representations (e.g. using the LEDGAR~\cite{tuggeneretal2020ledgar} dataset) or fine-tuned on large corpora such as the Harvward Law case corpus\footnote{https://case.law/}) with masked-language modelling or next-sentence prediction and tested on other legal downstream prediction tasks (such as in the CaseHOLD dataset~\cite{chalkidis2022lexglue} on tasks involving Overruling, Terms of Service, and CaseHOLD). 

%We highlight that retrieving the complete case (i.e. the combination of previous query, generated answer, and supporting evidence) creates opportunity to better personalise answers. 
%Furthermore, the retrieval is largely based on IR literature (i.e. given a query, return a snippet). We highlight the opportunities for CBR (i.e. given a query, what similar queries have been answered in the past) to incorporate reuse of best practice.

to make effective browsing of large IR collections, with knowledge-rich lattice constructs formed from 'most on-point cases~\cite{rissland1995hybrid}. 
highlighting how CBR was effectively employed to retrieve contextually relevant cases. 

%However, there are several complications with LLM-based applications operating in this domain. Legal text datasets (QA datasets withstanding) are often large unstructured corpora that require domain-expertise to comprehend and possess significant privacy concerns~\cite{lailaw2023large}. Additionally, LLMs themselves are black-box in operation, where explainability and interpretability remain an open challenge~\cite{lailaw2023large}. This becomes a problem as legal content is sensitive and requires proper citations to overcome hallucinations. 

\begin{figure}
    \centering
    \includegraphics[width=0.85\linewidth]{case_act_frequency_distribution.png}
    \caption{Legal act frequency distribution}
    \label{fig:case_act_frequency_distribution-label}
\end{figure}

\begin{table}[htbp]
\centering
\begin{tabular}{|c|c|p{0.5\linewidth}|}
\hline
\textbf{Index} & \textbf{Frequency} & \textbf{Act} \\ \hline
1 & 9 & Federal Court Rules \\ \hline
2 & 8 & Civil Aviation Regulations 1998 \\ \hline
3 & 8 & Land and Environment Court Act 1979 \\ \hline
4 & 7 & Corporations Act 2001 (Cth) \\ \hline
5 & 6 & Migration Act 1958 (Cth) \\ \hline
6 & 6 & Customs Act 1901, Customs Tariff Act 1995 \\ \hline
7 & 6 & Industrial Relations Act 1996 \\ \hline
8 & 5 & Environmental Planning and Assessment Act 1979 \\ \hline
9 & 5 & Trees (Disputes Between Neighbours) Act 2006 \\ \hline
10 & 5 & Migration Act 1958 \\ \hline
\end{tabular}
\caption{Indices, Frequencies, and Acts}
\label{tab:indices_frequencies_acts}
\end{table}

\subsection{Single-embedding Case Representation with BERT} 

Vanilla Bert first
todo: With Bert we have no dual embedding distinction because its not a metric learner; instead, we could mention that embeddings are learnt with self-supervised techniques like next-word or sentence prediction etc. 

legalBERT 

Given case $c_{\beta}$ we can extract the context for the prompt in two ways:
\begin{equation}
\text{Retrieved Result}, RR(\rho) = 
\begin{cases} 
S_{\beta} & \text{if } \rho = \text{"snippet-only"}, \\
(Q_{\beta}, S_{\beta}, A_{\beta}) & \text{if } \rho = \text{"case"}.
\end{cases}
\end{equation}

\begin{equation}
    \beta = \underset{c_i \in C}{\mathrm{argmax}} \, \; \text{Sim}(f(\mathcal{Q}), f(Q_i))
\end{equation}

\begin{equation}
    \beta = \underset{c_i \in C}{\mathrm{argmax}} \left( 
    w_1 \cdot \text{Sim}(f(\mathcal{Q}), f(Q_i)) +  
    w_2 \cdot \text{Sim}(g(\mathcal{Q}), g(S_i)) +  
    w_3 \cdot \text{Sim}(g(\mathcal{Q}), g(E_i) \right)
\end{equation}


 With intra-embedding retrieval, we use $\mathcal{Q}^L$ from a prompt to match query parts of the cases in the casebase.  
The best matching case identified from 
Intra-embedding retrieval is defined by:
\[
 \beta = \underset{c_i \in C}{\mathrm{argmax}} \, Sim(\mathcal{Q}^L, Q_i^L)
\]
Here, $\beta$ is the index of the best matching case, 
$Sim$ is a similarity metric (e.g., cosine similarity) that measures the similarity between the local embedding of the prompt's question and the local embeddings of the question parts of each case in the casebase.

With inter-embedding retrieval, we use the $\mathcal{Q}^G$ representation of the prompt query to search the casebase where case comparison is carried out as follows to identify the best matching case:
\[
\beta = \underset{c_i \in C}{\mathrm{argmax}} \, Sim(Q^G, S_i^G)
\]
where the focus is on adopting an information retrieval style of retrieval where attribute-to-ttribute matching is not strictly followed. 

Hybrid embedding is an alternative matching which involves a combination of both inter and intra-embeddings of the prompt's $\mathcal{Q}$ representations being used to match cases in a hybrid weighted retrieval approach to identify the best matching case:
\[
\beta = \underset{c_i \in C}{\mathrm{argmax}} \left( 
w1 \cdot \text{Sim}(\mathcal{Q}^L, Q^L_i) +  
w2 \cdot  \text{Sim}(\mathcal{Q}^G, S^G_i) +  
w3 \cdot  \text{Sim}(\mathcal{Q}^G, E_i^G) \right)

\]
Notice how both representation forms of the prompt's query $\mathcal{Q}^L$ and $\mathcal{Q}^G$ are used for retrieval. 

%Corpus - BLEU scores based on uni-grams were calculated to measure text overlap for all generated outputs, using the answer component of test instances as ground-truth.  Following~\cite{lin-och-2004-orange}, we added 1 to both the numerator and denominator to create an additive smoothing function. All recorded scores for the experiment were near zero, highlighting low overlap between the generated output and answer. Hybrid \abert with $k=1$ provided the best performance. %It is a significant 892.81\% improvement over the baseline.

\subsection{Qualitative Comparison}
\begin{table}[htbp]
\centering
\renewcommand{\arraystretch}{1.2}
\caption{Generated output comparison.}
\begin{tabular}{{p{0.12\linewidth} p{0.80\linewidth}}}
\toprule
\multicolumn{2}{c}{\textbf{Good Example}} \\
\midrule
Ground & The first case involved the appointment of provisional liquidators, Mr. Darren John Vardy and Mr. Terry Grant van der Velde, for a company named Darren Berry International Marine Pty Ltd (DBI) following an application by a creditor, Mr. Peter Carr. This appointment was made under Section 472(2) of the Corporations Act 2001 (Cth) after Mr. Carr had filed a winding up application that had not yet been determined. The court emphasized that the appointment of a provisional liquidator is a drastic remedy, but the law allows for a broad range of circumstances that might warrant its exercise, similar to the principles regarding the grant of urgent injunctive relief. The decision required a reasonable prospect that a winding up would ultimately be made and the balance of convenience must favor the making of the order. In contrast, the second case involved the approval of a scheme of arrangement between the plaintiff and the holders of ordinary shares in the plaintiff (excluding A.C.N. 614 507 247 Pty Ltd). This approval was granted pursuant to s 411(4)(b) of the Corporations Act 2001 (Cth). The court ordered an alteration to the definition of Excluded Shareholder in Schedule 1 of the scheme to specifically name A.C.N. 614 507 247 Pty Ltd. The plaintiff was also exempted from compliance with s 411(11) of the Act in relation to the Scheme, and was directed to lodge a copy of the approved Scheme with the Australian Securities and Investments Commission at the time of lodging a copy of these orders. The plaintiff and Superloop Limited intended to rely on the Court’s approval of the Scheme for the purpose of qualifying for exemption from the registration requirements of the US Securities Act of 1933. In summary, while both cases involved court orders under the Corporations Act 2001, they dealt with different aspects of corporate law: the first with the appointment of provisional liquidators in anticipation of a company winding up, and the second with the approval of a scheme of arrangement between a company and its shareholders. \\
Generated & In the case of the appointment of provisional liquidators for a company, the court order and reasons for judgment may include the following key differences from a scheme of arrangement case between a plaintiff and ordinary shareholders, with respect to costs: 1. Purpose and Nature of the Orders: The appointment of provisional liquidators is an interim measure taken by the court to protect the company's assets and prevent further harm to the creditors, usually when the company is insolvent or facing insolvency. In contrast, the approval of a scheme of arrangement is a consensual restructuring of a company's debt or equity, which requires the approval of the court and the affected stakeholders, including the ordinary shareholders. 2. Evidentiary Basis and Costs Assessment: In the appointment of provisional liquidators case, the court order and reasons for judgment will typically include an assessment of the costs incurred by the applicant, usually the company or creditors, to appoint the provisional liquidators. The applicant will provide an affidavit setting out the actual costs incurred and how they were calculated, along with evidence of the amount that is likely to be recovered on assessment. The court will apply a discount to assess the costs on a gross sum basis, using a broad brush approach to avoid the same level of detail as in a formal costs assessment. 3. Reasonableness and Proportionality: In the appointment of provisional liquidators case, the court will consider the reasonableness and proportionality of the costs incurred in the appointment process, taking into account the circumstances of the case, including the size and complexity of the company, the urgency of the situation, and the potential benefits to the creditors. 4. Costs Consequences: In the appointment of provisional liquidators case, the court may also consider the costs consequences for the parties involved. For instance, the company or the directors may be liable to pay the costs of the provisional liquidators if it is found that their conduct led to the company's insolvency. 5. Different Costs Regimes: In a scheme of arrangement case, the costs regime may be different, as the court will consider the costs consequences for the parties involved under the Companies Act or other relevant legislation. For instance, the ordinary shareholders may bear the costs of the scheme if it is approved by the court, or the costs may be allocated among the parties based on the terms of the scheme. 6. Different Legal Issues and Complexity: The legal issues and complexity in a scheme of arrangement case may be significantly different from an appointment of provisional liquidators case. The court will need to consider various legal and factual issues, including the terms of the scheme, the consequences for the various stakeholders, and the impact on the company's financial position. The costs assessment in a scheme of arrangement case may be more complex and detailed than in an appointment of provisional liquidators case.\\
\midrule
\multicolumn{2}{c}{\textbf{Bad Example}} \\
\midrule
Ground & In the case of Orkun James Sen v Doors Plus Pty Limited there is no clear outcome of the unfair dismissal application. The matter was referred to the Commission by the Industrial Registrar pursuant to Practice Direction 17 and that the applicant, Mr. Sen, had sent a letter to the Industrial Registrar on 2nd March 2006. On the other hand, in the case of Peter Blum v Global Vision International Pty Ltd, the application for relief from unfair dismissal was refused. The termination was not considered harsh, reasonable, or unjust. This conclusion was reached following a hearing on 10th October 2001, and the judgment was delivered on 16th November 2001. Therefore, the outcomes of the two cases were different, with the latter resulting in a clear refusal of the application for relief from unfair dismissal.\\
Generated & In the context of the Industrial Relations Commission of New South Wales, the outcomes of the unfair dismissal applications differed in the cases of Orkun James Sen v Doors Plus Pty Limited and Peter Blum v Global Vision International Pty Ltd. In the case of Orkun James Sen v Doors Plus Pty Limited [2011] NSWIRComm 781 (16 August 2011), the Commission found that the dismissal was harsh, unjust or unreasonable. The employee was awarded compensation for the financial loss he suffered as a result of his dismissal. In contrast, in the case of Peter Blum v Global Vision International Pty Ltd [2011] NSWIRComm 888 (2 September 2011), the Commission found that the dismissal was not unfair. The employee did not receive any compensation. These outcomes differed because in the Sen case, the Commission found that the dismissal was harsh, unjust or unreasonable based on the evidence presented. In contrast, in the Blum case, the Commission found that the dismissal was fair based on the evidence presented. Therefore, the outcomes of the unfair dismissal applications differed in terms of the compensation awarded to the employees. In the Sen case, the employee received compensation, while in the Blum case, he did not.\\
